Hermitian Yang-Mills metrics on reflexive sheaves over asymptotically cylindrical K\"ahler manifolds

We prove an analogue of the Donaldson-Uhlenbeck-Yau theorem for asymptotically cylindrical K\"ahler manifolds: If $\mathscr{E}$ is a reflexive sheaf over an ACyl K\"ahler manifold, which is asymptotic to a $\mu$-stable holomorphic vector bundle, then it admits an asymptotically translation-invariant protectively Hermitian Yang-Mills metrics (with curvature in $L^2_{\mathrm{loc}}$ across the singular set). Our proof combines the analytic continuity method of Uhlenbeck and Yau [UY86] with the geometric regularization scheme introduced by Bando and Siu [BS94].

==> CkEstimate.tex <==
\section{Bando--Siu interior \texorpdfstring{$C^k$}{Ck} estimate}
\label{Sec_InteriorEstimates}

\begin{theorem}[{\citet[Proposition 1]{Bando1994}}]
  \label{Thm_CkBounds}
  Let $(X,g,I)$ be a Kähler manifold with bounded geometry and let $\sE$ be a holomorphic vector bundle over $X$.
  If $H_0$ and $H$ are Hermitian metrics on $\sE$ related by
  \begin{equation*}
    H = H_0 e^s
  \end{equation*}
  for $s \in C^\infty(X,i\su(\sE,H_0))$,
  then
  \begin{equation*}
    r^k\Abs{\nabla_{H_0}^k s}_{C^k(B_r(x))}
    \leq c_k\epsilon_k\(\Abs{s}_{L^\infty(B_{2r}(x))} + \Abs{K_{H}}_{L^\infty(B_{2r}(x))}\)
  \end{equation*}
  where $c_k$ depends only on $H_0$ and the geometry of $X$,
  and $\epsilon_k$ is a smooth function which vanishes at the origin.
\end{theorem}

It suffices to prove this in the case where $H_0$ is a flat metric on a trivial holomorphic bundle over $\bar B_2 \subset \C^n$.
The theorem is not a straight-forward consequence of standard bootstrapping techniques because we only have
\begin{equation*}
  \Delta s
  = A(K_H) + C(\nabla s \otimes \nabla s)
\end{equation*}
where $A$ and $C$ are linear with coefficients depending on $s$;
see \autoref{Prop_KH0ExpS}.
The usual Sobolev estimates will not suffice to prove \autoref{Thm_CkBounds} without any control of $\nabla s$.
However, if we assume $C^{0,\beta}$ bounds on $\nabla s$ of the above form, then the usual method does give the desired estimates.
It is well known to analysts that for an equation of this form $C^{0,\beta}$ bounds on $\nabla s$ can be obtained provided a bound on the Morrey norm $\Abs{\nabla s}_{L^{2,2n-2+2\alpha}}$;
see \autoref{Def_Morrey}.
We give full details for this fact, which is completely general and has nothing to do with Hermitian Yang--Mills metrics, in \autoref{Sec_Hildebrandt}.
All of this being said, it thus suffices to prove the following proposition.

\bigbreak

\begin{prop}
  Denote by $H_0$ a flat Hermitian metric on the trivial holomorphic bundle of rank $r$ over $\bar B_2 \subset \C^n$.
  If $H = H_0e^s$ with $s \in C^\infty(\bar B_2,i\su(r))$, then
  \begin{align*}
    [s]_{C^{0,\alpha}(\bar B_1)}
    &\lesssim
      \Abs{\nabla s}_{L^{2,2n-2+2\alpha}(B_1)}\\
    &\leq
      \epsilon(\Abs{s}_{L^\infty(B_2)}+\Abs{K_H}_{L^\infty(B_2)})
  \end{align*}
  where $\alpha \in (0,1)$ is depends on $\Abs{s}_{L^\infty(B_2)}$ in a monotonely decreasing way,
  and $\epsilon$ is a smooth function which vanishes at the origin.
\end{prop}

\begin{proof}
  For $x \in B_{1}$ define $f_x \co (0,1] \to [0,\infty)$ by
  \begin{equation*}
    f_x(r) := \int_{B_r(x)} G_x \abs{\nabla s}^2
  \end{equation*}
  with $G_x(\cdot) := \abs{\cdot-x}^{2-2n}$.
  We will show that
  \begin{equation*}
    f_x(r) \leq \epsilon r^{2\alpha}
  \end{equation*}
  with $\epsilon$ and $\alpha$ as in the proposition.
  This implies the asserted Morrey bound.

  In the following we fix $x \in B_1$ and $r \in (0,1/2]$ and omit writing the subscript $x$ to simplify notation.

  \setcounter{step}{0}
  \begin{step}
    We have $f(r) \leq \epsilon$.
  \end{step}

  Fix a smooth function $\chi \co [0,\infty) \to [0,1]$ which is equal to one on $[0,1]$ and vanishes outside $[0,2]$.
  Set $\chi_{r}(\cdot) := \chi(\abs{\cdot - x}/r)$.
  Using we have
  \begin{equation*}
    \abs{\nabla s}^2
    \lesssim
      \epsilon\cdot(1-\Delta\abs{s}^2),
  \end{equation*}
  which follows from \eqref{Eq_NablaS}, we compute
  \begin{align*}
    f(r) 
    &\leq
      \int_{B_{2r}(x)} \chi_{r} G \cdot \abs{\nabla s}^2 \\
    &\lesssim
      \epsilon\int_{B_{2r}(x)} \chi_{r} G \cdot (-\Delta\abs{s}^2)
      + \chi_{r} G \\
    &\lesssim
      \epsilon r^{-n} \int_{B_{2r}(x)\setminus B_{r}(x)} \abs{s}^2
      + \epsilon r^2 \\
    &\leq \epsilon.
  \end{align*}
  Here we used the convention of ``generic constants''; that is, $\epsilon$ is allowed to increase from one line to the next.

  \begin{step}
    We have $f(r) \leq \gamma f(2r) + \epsilon r^2$ for some constant $\gamma \in (0,1)$ depending on $\|s\|_{L^\infty(B_2)}$.
  \end{step}
  
  Set
  \begin{equation*}
    \bar s := \fint_{B_{2r}(x)\setminus B_r(x)} s \in i\su(r) \qandq \sigma := \log(e^{s}e^{-\bar s}).
  \end{equation*}
  Observe that
  \begin{equation*}
    \abs{\nabla s}^2
    \lesssim
    M\abs{\nabla\sigma}^2
    \qandq
    |\sigma|^2
    \lesssim
      M\abs{s-\bar s}^2
  \end{equation*}
  with $M>0$ some constant depending on $\Abs{s}_{L^\infty(B_2)}$ in a monotonely increasing way.
  Arguing as in the previous step we have
  \begin{equation*}
    \abs{\nabla \sigma}^2 
    \leq
      M\(-4\inner{K_{H}}{\sigma} - \Delta\abs{\sigma}^2\)
    \leq
      M(1 - \Delta\abs{\sigma}^2).
  \end{equation*}
  Using the above and Poincaré's inequality we have
  \begin{align*}
    \int_{B_r(x)} G\abs{\nabla s}^2
    &\lesssim
      M^2\int_{B_{2r}(x)} \chi_r G\cdot (-\Delta\abs{\sigma}^2)
      + \epsilon \chi_r G \\
    &\lesssim
      M^2\cdot r^{-2n} \int_{B_{2r}(x)\setminus B_r(x)} \abs{\sigma}^2
      + \epsilon r^2 \\
    &\lesssim
      M^3\cdot r^{-2n} \int_{B_{2r}(x)\setminus B_r(x)} \abs{s-\bar s}^2
      + \epsilon r^2 \\
    &\lesssim
      M^3 \cdot r^{2-2n} \int_{B_{2r}(x)\setminus B_r(x)} \abs{\nabla s}^2
      + \epsilon r^2 \\
    &\lesssim
      M^3\int_{B_{2r}(x)\setminus B_r(x)} G\abs{\nabla s}^2
      + \epsilon r^2.
  \end{align*}
  This gives the asserted inequality.

  \begin{step}
    We have $f(r) \leq \epsilon r^{2\alpha}$.
  \end{step}

  We can assume that $\gamma \geq 1/2$.
  Set $g(r) := f(r) + \frac{c}{4\gamma-1}\epsilon r^2$.
  By the second step
  \begin{equation*}
    g(r)
    \leq \gamma^k g(2^kr).
  \end{equation*}
  Setting $k := \log_2 \ceil{1/2r}$, we have $\gamma^k \lesssim r^{2\alpha}$ for some $\alpha \in (0,1)$ depending only on $\gamma$;
  hence, by the first step
  \begin{equation*}
    f(r) \leq \epsilon r^{2\alpha}.
    \qedhere
  \end{equation*}
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ACylDUY"
%%% End:


==> aux/colors.tex <==
\usepackage{multicol, color}

\definecolor{gold}{rgb}{0.85,.66,0}
\definecolor{cherry}{rgb}{0.9,.1,.2}
\definecolor{burgundy}{rgb}{0.8,.2,.2}
\definecolor{orangered}{rgb}{0.85,.3,0}
\definecolor{orange}{rgb}{0.85,.4,0}
\definecolor{olive}{rgb}{.45,.4,0}
\definecolor{lime}{rgb}{.6,.9,0}
%\definecolor{green}{rgb}{.3,.5,0}
\definecolor{green}{rgb}{.2,.7,0}
\definecolor{grey}{rgb}{.4,.4,.2}
\definecolor{brown}{rgb}{.4,.3,.1}
\def\gold#1{\textcolor{gold}{#1}}
\def\cherry#1{\textcolor{cherry}{#1}}
\def\burgundy#1{\textcolor{burgundy}{#1}}
\def\orange#1{\textcolor{orange}{#1}}
\def\orangered#1{\textcolor{orangered}{#1}}
\def\olive#1{\textcolor{olive}{#1}}
\def\lime#1{\textcolor{lime}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\grey#1{\textcolor{grey}{#1}}
\def\brown#1{\textcolor{brown}{#1}}


==> aux/conf.tex <==
\newif\ifpaper
\newif\ifarxiv

\paperfalse
\arxivfalse


==> aux/init.tex <==
\usepackage{etoolbox}
\newtoggle{arXiv}
\newtoggle{screen}

==> aux/solarized.tex <==
%%%%%%%%%%%%
\usepackage{xcolor}
% Solarized palette
\definecolor{Base03}{HTML}{002B36}
\definecolor{Base02}{HTML}{073642}
\definecolor{Base01}{HTML}{586e75}
\definecolor{Base00}{HTML}{657b83}
\definecolor{Base0}{HTML}{839496}
\definecolor{Base1}{HTML}{93a1a1}
\definecolor{Base2}{HTML}{EEE8D5}
\definecolor{Base3}{HTML}{FDF6E3}
\definecolor{Yellow}{HTML}{B58900}
\definecolor{Orange}{HTML}{CB4B16}
\definecolor{Red}{HTML}{DC322F}
\definecolor{Magenta}{HTML}{D33682}
\definecolor{Violet}{HTML}{6C71C4}
\definecolor{Blue}{HTML}{268BD2}
\definecolor{Cyan}{HTML}{2AA198}
\definecolor{Green}{HTML}{859900}
%
\def\grey#1{\textcolor{Base0}{#1}}
\def\blue#1{\textcolor{Blue}{#1}}
\def\red#1{\textcolor{Red}{#1}}
\def\magenta#1{\textcolor{Magenta}{#1}}
\def\violet#1{\textcolor{Violet}{#1}}
\def\orange#1{\textcolor{Orange}{#1}}
\def\yellow#1{\textcolor{Yellow}{#1}}
\def\green#1{\textcolor{Green}{#1}}
\def\cyan#1{\textcolor{Cyan}{#1}}
%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

